Exploiting Ergonomic Priors in Human-to-Robot Task Transfer

In recent years, there has been a booming shift in the development of versatile, autonomous robots by introducing means to intuitively teach robots task-oriented behaviour by demonstration. In this paper, a method based on programming by demonstration is proposed to learn null space policies from constrained motion data. The main advantage to using this is generalisation of a task by retargeting a systems redundancy as well as the capability to fully replace an entire system with another of varying link number and lengths while still accurately repeating a task subject to the same constraints. The effectiveness of the method has been demonstrated in a 3-link simulation and a real world experiment using a human subject as the demonstrator and is verified through task reproduction on a 7DoF physical robot. In simulation, the method works accurately with even as little as five data points producing errors less than 10^-14. The approach is shown to outperform the current state-of-the-art approach in a simulated 3DoF robot manipulator control problem where motions are reproduced using learnt constraints. Retargeting of a systems null space component is also demonstrated in a task where controlling how redundancy is resolved allows for obstacle avoidance. Finally, the approach is verified in a real world experiment using demonstrations from a human subject where the learnt task space trajectory is transferred onto a 7DoF physical robot of a different embodiment.

==> ext/Makefile <==
SHELL := /bin/bash
SUBDIRS := $(subst Makefile,,$(wildcard */Makefile))
CLEANDIRS = $(SUBDIRS:%=clean-%)

default: \
	tex/abbreviations.tex \
	tex/symbols.tex \
	subdirs 

clean: cleandirs

subdirs: $(SUBDIRS)

#tex/%.tex: 
#	[[ -d $@ ]] || svn export -r 46 svn+ssh://kcl/home/k1217511/svnroot/Templates/Tex/Global/$(subst tex/,,$@) $@
tex/abbreviations.tex: 
	[[ -d $@ ]] || svn export -r 47 svn+ssh://kcl/home/k1217511/svnroot/Templates/Tex/Global/$(subst tex/,,$@) $@
tex/symbols.tex:
	[[ -d $@ ]] || svn export -r 47 svn+ssh://kcl/home/k1217511/svnroot/Templates/Tex/Global/$(subst tex/,,$@) $@

$(SUBDIRS):
	 $(MAKE) -C $@

cleandirs: $(CLEANDIRS)
$(CLEANDIRS): 
	$(MAKE) -C $(@:clean-%=%) clean

.PHONY: subdirs $(SUBDIRS)
.PHONY: cleandirs $(CLEANDIRS)



==> tex/method.tex <==
\section{Materials and Methods}\label{s:method}
\noindent The aim of this paper is to evaluate Constraint Consistent Learning \cite{jeevan2017learningFast,learningspaceLin,dependantLearning2016,Howard2009} as a means to adapt human-ergonomic demonstrations for use with a robotic controller, by \il{\item learning the task constraints present in a demonstration, and \item using these to replace the secondary (human ergonomic) features of behaviour with a control strategy more suited to the robot}. The procedure is as follows. \mh{Why is CCL the right approach? Needs to be argued much more strongly both here, and in \sref{introduction} and \sref{problem_definition}.}
%In this paper, the use of the proposed approach is recommended over the more simple and sub-optimal control policy of directly copying the user, as our method forms an estimate of the task space constraint matrix $\bA$ to be used in $\bpi$ to manipulate systems away from singular points while performing a task. This minimises the risk of encountering singularities which lead to unpredictable behaviour.

%\noindent In this paper, the use of the proposed approach is recommended over the more simple and sub-optimal control policy of directly copying the user, as our method forms an estimate of the task space constraint matrix $\bA$ to be used in $\bpi$ to manipulate systems away from singular points while performing a task. This minimises the risk of encountering singularities which lead to unpredictable behaviour.

\subsection{Data Collection}\label{s:representationOfData}
\noindent The data is assumed to consist of $\Nd$ pairs of observed states $\bxn\in\R^\dimx$ and actions $\bun\in\R^\dimu$ collected though ergonomic demonstrations of the primary task performed by a human demonstrator. \mh{Bearing in mind the discussion about ergonomics in preceding sections, what restrictions are there on what $\bx$ and $\bu$ could be in this paper? Can they only be joint angles/velocities? Are they strictly observations from natural behaviour/motion capture (\ie not kinesthetic demonstrations)?} 

\subsection{Task Priority Decomposition} \label{s:taskPioritisedConstraints}
\noindent The control policy from which the demonstration data derives is assumed to consist of distinct prioritised components encoding \emph{task-oriented} and \emph{secondary} (\ie \emph{ergonomics-oriented}) parts
\begin{align}
\bu(\bx)&= \buts(\bx)+\buns(\bx)\\
        &=\bA^\dagger(\bx)\bb(\bx)+\bN(\bx)\bpi(\bx)
\label{e:problem-solution}
\end{align}
where $\buts$ and $\buns$ are the task-critical and secondary components, respectively,  $\bx\in\R^\dimx$ represents state and $\bu\in\R^\dimu$ the action. 

The task-oriented component derives from a set of $\dimb$-dimensional task-constraints
\begin{equation}
  \bA(\bx)\bu(\bx)=\bb(\bx)
  \label{e:problem-constraint}
\end{equation}
where %$\bx\in\R^\dimx$ represents state% (usually represented either in end-effector or joint space), 
$\bA(\bx)\in\R^{\dimb\times\dimu}$ is a matrix describing the constraints, and $\bb(\bx)\in\R^{\dimb}$ is the \emph{task space policy} describing the primary task to be accomplished. {\color{mh}For instance, in the drawer opening example, the policy $\bb(\bx)$ may be described by [...]} \mh{What?} It is assumed that the $\bA(\bx)$ should be learnt by the robot through demonstrations. \mh{Why?} %while also autonomously handling the degree of constrainedness of the system such that it enhances the flexibility.
%
%The general solution to \eref{problem-constraint} is given by % Learning $\bA$ only given $\bu$ is possible as shown below by inverting \eref{problem-constraint} 
%\begin{equation}
%	\bu(\bx) = \underbrace{\bA^\dagger(\bx)\bb(\bx)}_{\buts}+ \underbrace{\bN(\bx)\bpi(\bx)}_{\buns}
%\label{e:problem-solution}
%\end{equation}
%where $\buts$ is the task space component that implements the task space policy, $\buns$ is the null space component and 

The secondary component is composed of two parts, namely, a policy $\bpi(\bx)$ and the projection matrix
\begin{equation}
	\bN(\bx)=\I-\bA(\bx)^\dagger\bA(\bx)\in\R^{\dimu\times\dimu}
	\label{e:N}
\end{equation}
Here, $\I\in\R^{\dimu\times\dimu}$ denotes the identity matrix and $\bA^\dagger=\bA^\T(\bA\bA^\T)^{-1}$ is the Moore-Penrose pseudo-inverse of $\bA$. In the context of human task-oriented behaviour, $\bpi(\bx)$ captures the part of the demonstrated movement that aims to bring the body into an ergonomic posture, while $\bN(\bx)$ ensures that such actions do not conflict with the task-oriented component of behaviour (by projecting $\bpi(\bx)$ onto the null space of $\bA$). The key to the proposed approach is the identification of the latter component of movement in the demonstrations, such that it can be replaced by an alternative controller, $\bpir(\bx)$, better suited to the needs of the robotic imitator. 



% Commonly, in the context of programming by demonstration by non-expert users, $\bA, \bN, \bb$ and $\bpi$ are not explicitly known. Instead, the controller must be derived from data. In this paper, it is assumed that data is given as pairs of $\Nd$ observed states $\bx_n$ and actions $\bu_n$.

%What non-expert users may not be aware of is that $\buns$ controls the additional free non-task related degrees of freedom of the system. It can be thought of as a lower priority task which does not conflict with the goal defined in the task space component. The benefit of having a null space component is evident in tasks which have multiple solutions. For example, a reaching task where multiple paths to a goal may be available, some paths may drive a system closer to its joint limits or singular configurations which can lead to an increased risk of  getting stuck or cause turbulent movement in face of perturbations or the imposition of additional constraints.

Throughout the following it is assumed that \il{\item observations are in the form presented in \eref{problem-solution}, \item $\bb$ from the task space varies throughout all observations, \item $\bpi$ is consistent throughout $\bu$% and is performed in a way that is comfortable/ergonomic for the user
, %\item the ergonomic observations within the null space can be assessed using the reduced RULA (\fref{reducedRulaImage}) in order to differentiate between the demonstrators' and systems' comfort 
and \item $\bA$, $\bN$, $\bb$, and $\bpi$ are not explicitly known for any given observation}.
\mh{Is it necessary to assume $\bA$, $\bN$ and $\bpi$ are unknown in this context? What happens if you know them?}


\subsection{Identifying the Components and Constraints}\label{s:learningComponentAndConstraint}
\noindent To find the parts of the movement corresponding to human-ergonomic behaviour--and therefore suitable for replacement by a robot-specific controller--two steps are needed: \il{\item separation of the task-oriented and secondary components of the observed actions, and \item estimation of $\bA$ (and thereby $\bN$) for purposes of replacing $\bpi(\bx)$}. 

\subsubsection{Separating Task-oriented and Secondary Components}\label{s:separatingNullspaceComponent}
Separation of the two components can be achieved through the approach first proposed in \cite{towell2010learning}. As shown there, the first and second terms of \eref{problem-solution} can be separated by seeking an estimate $\ebuns$ that minimises
\begin{equation}
  E[\ebuns] = ||\estimated{\mathbf{P}}_\nd\bun - \ebunsn||^2
  \label{e:learningnullspacecomponent}
\end{equation}
where $\ebunsn := \ebuns(\bxn)$ and $\estimated{\mathbf{P}}_\nd := {\ebunsn\ebunsn}^\T / ||\ebunsn||^2$. This works on the principal that, there exists a projection $\mathbf{P}$ for which $\mathbf{P}\bu = \mathbf{P}(\buts + \buns) = \buns$. Similarly, an estimate of $\ebuts$ can be made by subtracting the estimated $\ebuns$ from $\bu$, \ie $\ebuts=\bu-\ebuns$.


\subsubsection{Representing \& Learning the Constraint $\bA$}\label{s:learningTheConstraint}\label{s:RepresentationOfA}
\noindent Given the estimates of $\bv$ and $\bw$, the next step is to form an estimate $\bA$ (or, equivalently, $\bN$) in order that the secondary policy for the robot, $\bpir$, can be safely added to the robot control without fear of it interfering with the task-oriented movement. 

To this end, $\bA$ is estimated following the approach first proposed in 
\cite{learningspaceLin}. Here, the constraint matrix is represented in the form
\begin{equation}
	\bA(\bx) = \bLambda \bPhi(\bx)
	\label{e:A-matrix}
\end{equation}
where $\bLambda\in\R^{\dimb\times\dimPhi}$ is an unknown selection matrix (to be estimated in the learning) and $\bPhi(\bx)\in\R^{\dimPhi\times\dimu}$ is a feature matrix. The rows of the latter contain candidate constraints that can be predefined where there is prior knowledge of potential constraints affecting the user, or can take generic forms such as a series of polynomials. For example, one may choose $\bPhi(\bx)=\bJ(\bx)$, the Jacobian modelled after the demonstrators arm, where $\bA(\bx)=\bLambda\bJ(\bx)$ encodes constraints on the motion of specific degrees of freedom in the end-effector space.

Several learning methods are available for estimating the selection matrix $\ebLambda$ \cite{dependantLearning2016,lin2015learning,armesto2017efficientlearning}. in this paper, the estimate is formed by minimising
\begin{equation}
  E[\estimated{\bA}] =  \sum_{\nd=1}^\Nd \ebunsn^\T(\ebLambda\bPhi_\nd)^{\dagger}\ebLambda\bPhi_\nd\ebunsn
  \label{e:learninglambda}
\end{equation}
where $\bPhi_\nd:=\bPhi(\bxn)$. This results in the estimate $\ebA(\bx)=\ebLambda\bPhi(\bx)$.

\subsection{Robot-ergonomic Controller}
\noindent The final stage is to replace the human-ergonomic secondary control policy with a robot-specific one, while maintaining the same task-oriented movements. For this, a control policy of the form
\begin{align}
	\bur(\bx)= \ebuts(\bx)+\ebN(\bx)\bpir(\bx)
	\label{e:robot-controller}
\end{align}
\mh{Potentially, it may be better to use $\pinv{\ebA}\ebuts$ than just $\ebuts$, as this will ensure orthogonality between the two components.}
is used, where $\ebuts$ is the estimated task-oriented component of movement and $\ebN$ is the estimated null-space projection matrix. As noted in \sref{taskPioritisedConstraints}, $\bpir$ can be chosen according to the needs of the robotic system. {\color{mh}For example, [...]} \mh{What are potential choices? Why would they be suitable?} 

A particularly suitable choice \mh{Why?} is to use a policy that avoids singular postures. Following \cite{learningSingularityAvoidanceJeevan2019}, the estimated constraint matrix $\ebA$, can be used to form an \textit{estimate of the system manipulability} \cite{Yoshikawa} for any configuration within the support of the data
\begin{equation}
  \ev(\bx) = \sqrt{\det\left(\ebA(\bx)\ebA(\bx)^\T\right)}.
  \label{e:manipulability-index-with-eA}
\end{equation}
The latter can be used to drive the system away from singular points, thereby reducing the risk of unpredictable behaviour. The simplest approach to doing this is to apply a gradient-based control policy
\begin{equation}
  \bpir(\bx) = \nabla_\bx\ev.
  \label{e:v cost function}
\end{equation}
%Alternatively, if the task space trajectory is predictable, $\ev$ can be used in combination with global approximation in the null space (see, \eg \cite{nakamura1991advanced}). 
%
%Replacement of the null space component to better suit the system, while also maintaining the humans task-oriented behaviour in the task space component blends the human and robot control schemes for each part of the equation \eref{problem-solution} and should lead to improved mean performance as supported by \cite{frameworkForTeachingImpedanceBehaviourYuchen}.
\begin{figure}[t!]
    \vspace{1mm}
      \centering
      \framebox{\parbox{3in}{}
      %\def\svgwidth{.85\columnwidth}
      %\input{images/hosePlan2.eps_tex}
      %\includegraphics[scale=1.0]{images/unconstrainted_2x2_jacobian.eps}
      \includegraphics[width=0.45\textwidth]{images/Plan3.png}}
	  \caption{Overview of approach to maximising manipulability in \PbD tasks. (A) Motion data is collected through ergonomic demonstrations of the task. (B1) The data is used to determine the separate task and null space components so that (B2) the latter can be used to estimate the constraint. (C) Using the estimated constraint matrix, an estimate of the constrained manipulability $\ev$ is made. (D) This estimate is used to select states with greater manipulability, and (E) control the robot toward these when performing the primary task.}
      \label{f:plan}
\end{figure}
\fref{plan} shows a brief overview of the major steps involved in the proposed approach.
\mh{On balance, I think you can keep \fref{plan}, if you ensure that (i) it is updated according to the new message of the paper (ii) it is made to look sufficiently different from the figure in the IROS paper.}

% \subsection{Evaluation Criteria for Method Performance}
% \noindent To compare how well suited the proposed approach is in contrast to directly mimicking the ergonomic demonstrations of the user, on the ergonomic side the RULA worksheet (\fref{reducedRulaImage}) is suggested, whereas, \eref{manipulability-index-with-eA} is used for the assessment of the manipulability.
% 
% Learning the constrained manipulability may not always be a trivial matter depending on the task at hand. Factors such as, high dimensionality of a system, or the structure of particular constraints in comparison to others, can lead to poor learning performance. It is therefore necessary to define a metric to assess learning performance.
% 
% The Normalised Manipulability Index Error (NMIE) evaluates the fitness of the learnt manipulability index $\ev$, and measures the distance between the true and learnt manipulability index
%
% \begin{equation}\label{NMIE}
% 	E_{NMIE} =
% 	%\frac{1}{\mathcal{N}\sigma_\mathbf{u}^2}
% 	\frac{1}{\mathcal{N}\sigma_\mathbf{\v}^2} \sum_{n=1}^{\mathcal{N}}||\mathbf{\v}_n - \mathbf{\ev}_n ||^2
% \end{equation}
%
%\noindent where $\mathcal{N}$ is the number of data points. The error is normalised by the variance of $\mathbf{\v}$. The MIE will reach zero as $\mathbf{\ev}\to\mathbf{\v}$.
%
%\jm{\done{\atMH:\sref{method} is to do.}}

\mh{At the moment, the theoretical contribution of this paper is rather minor (it's more or less \cite{frameworkForTeachingImpedanceBehaviourYuchen} applied to kinematics instead of impedance control). This is a concerning weakness. To strengthen it, I think it would be valuable to give some deeper thought as to what can be leveraged from the problem context, and adapt the theory accordingly. For example, (i) is it reasonable to assume $\bA$ is totally unknown? You usually know that, for example, drawers open horizontally, hence knowledge of this could be used, and might help with the robustness of learning. (ii) You argue that people use a stereotypical $\bpi$, \ie RULA, in their movements. Therefore, is it reasonable to assume $\bpi$ is totally unknown? Perhaps assuming knowledge of $\bpi$ could lead to better results, and new theoretical insights.}

==> tex/problem_definition.tex <==
\section{Problem Definition}\label{s:problem_definition}
\noindent The aim of this work is to examine how human-ergonomic features of task-oriented demonstrations can be taken into account in the context of robotic imitation learning, such that the resultant behaviours are \emph{optimised to the robot's embodiment}.


\subsection{Human-ergonomic Demonstrations} \label{s:humanErgonomicsRULA}
\noindent In most scenarios where ordinary people are asked to provide natural demonstrations of a given task, in the absence of external constraints, it can generally be assumed the behaviour observed will be optimised for efficiency and comfort according to their embodiment. This means that postures adopted by the user in the course of a demonstration are likely to show stereotypical traits that promote these goals. For example, when reaching to a target such as a drawer handle, typically people will adopt a low-energy posture with little limb flexion, thereby minimising the effort needed to counter gravity (see \fref{staticPosture}). This is further encouraged by the arrangement of objects in human work-spaces, that are also designed to maximally promote the comfort of their occupants. In the aforementioned example, the location of the drawer handle, and its path during opening, are configured to minimise the need for deviation from this posture. 

Such interactions of humans with their environment have long been studied in the field of \emph{human ergonomics} \cite{realtimeergonomicsAli,ergonomicsOfficeTraining}, with a view to improving and optimising the design of workspaces. As part of this, a number of measures exist that aim to quantify good design and working practice which assess various exposure factors such as posture, force and movement frequency to name a few \cite{ergonomicMethods}. In monitoring posture for manual tasks, for example, a popular system is the \newabbreviation{\RULA}{RULA} \cite{rulaMethod} that works by scoring static poses of individual joints of the upper limb, where an overall lower score implies that the posture is more ergonomic, and assessing the effect of repeated actions. For reference, a reduced version of the RULA worksheet adapted from that of ErgonomicsPlus\textsuperscript{\textcopyright} is shown in \fref{reducedRulaImage}. Several other measures can also be used to categorically assess risk in static poses such as the Loading on the Upper Body Assessment (LUBA) or New Ergonomic Posture Assessment (NERPA), however studies show that out of these RULA performs best in assessing the risk factor of postures that incite muscle fatigue and discomfort which can lead to work-related musculoskeletal disorders \cite{compareThreeErgonomicMethods}.

\begin{figure}[t!]
	\centering%
	\includegraphics[width=\linewidth]{images/staticPostureRULAManiV2.png}
	\caption{Typical drawer-opening posture that is ergonomic for humans but not for robots. According to \RULA, the posture shown has a relatively good score of $2$ (upper arm position = $-70\degree$ $\rightarrow$ upper arm score 1, lower arm position = $0\degree$ $\rightarrow$ lower-arm score $2$ and wrist = $0\degree$ $\rightarrow$ wrist score $1$, see \fref{reducedRulaImage}). However, for inverse kinematics control in a robotic system, this pose is singular (manipulability score $0$), and therefore unlikely to meet the task demands.}
	\label{f:staticPosture}
\end{figure}
\mh{Please remove the large title text from \fref{staticPosture}.}

% Rapid Upper Limb Assessment (RULA) can be used as an approximate measure of this. 
%\noindent The posture monitoring method RULA aims to improve the human’s ergonomic state by optimising the interactions based entirely on the human’s comfort and ergonomics \cite{realtimeergonomicsAli}. 
\begin{figure}[t!]
	\centering%
	\includegraphics[width=0.48\textwidth]{images/reducedRulaV3.png}
	\caption{Reduced version of the Rapid Upper Limb Assessment (RULA) worksheet which focuses the ergonomics assessment to a 2D lateral perspective (arm/wrist analysis only without bending from the midline or twisting). This is adapted from \cite{rulaguide2019}. To compute the score for any static pose, follow steps 1-3 successively so that three individual scores are obtained for the upper arm, lower arm and wrist, respectively. Then, enter those individual scores into the table 'Scores' (on the right) where the upper arm and lower arm are used in turn to select the appropriate row and the wrist score selects the correct column resulting in a final score which can be checked against the 'Scoring' box below the table to verify whether it is an acceptable posture or may require change. See \fref{reducedRulaImage} for an example on a static posture.}
	\label{f:reducedRulaImage}
\end{figure}  
%\jm{\done{\atMH:I do not understand the arrows in \fref{reducedRulaImage}. Also, perhaps you can remove the text ``Step 3a: Adjust [...]''. Do you have a reference for this figure?}}
%A reduced version of the RULA worksheet adapted based on the works by ErgonomicsPlus\textsuperscript{\textcopyright} is presented here in \fref{reducedRulaImage} for reference throughout the paper. This version cuts out the assessing of movements which cannot be effectively captured outside of the 2D lateral view of the subject and focuses on the upper arm, lower arm and wrist which provides sufficient data for evaluation between RULA and manipulability. It works by scoring static poses where an overall lower score implies that the posture is more ergonomic. While scoring is performed on a static posture, the posture itself does not have to be constant as metrics are provided for strain such as assessing repeated actions which is out of the scope of this paper. 
\jm{\done{\atMH:Please use the caption of \fref{reducedRulaImage} to explain how the score is computed.}}
\mh{What about accessibility (\eg if there is an obstacle in front of the drawers, the user/robot might need to reach over in a non-ergonomic way)?}

\subsection{Robot Imitation of Ergonomic Behaviours}\label{s:robotErgonomics}
\noindent While working practices and environments that promote ergonomic postures can lead to greater efficiency in humans, the same cannot be said for robotic systems tasked with entering those same environments and performing similar tasks. It has long been established that the differences in embodiment between humans and robots, including the kinematic structure \cite{Alissandrakis2007} and dynamics \cite{Howard2013a} mean that direct imitation of human behaviour is suboptimal. 

In the context of postural imitation of human ergonomic behaviour, this issue is particularly pronounced. For instance, considering the drawer-opening example, while the posture shown in \fref{staticPosture} scores well in terms of human ergonomics (RULA score: 2 points, considered an acceptable posture), the same is not true for a robot imitator. In this case, because the arm is fully extended, this posture represents a singular pose for standard robotic inverse kinematics controllers, which can lead to unpredictable and potentially dangerous behaviour. Conversely, a pose in which the upper arm is flexed to be parallel with the horizontal would be a high-stress pose for a human (and therefore score proportionately worse by \RULA), but may not be a difficult posture for a robot with low back-drivability to maintain, since its joints can effectively be locked in place with no energy cost. 

%This is further highlighted by the manipulability measure where the orientation of the base does not contribute to its score, meaning that with respect to a system modelled after the arm with the base being attached parallel to the shoulder, the upper arm can rotate freely with manipulability score will staying as 0 unlike in the case of the RULA assessment. \jm{\atMH Partially done \atJM This is not very convincing, as it seems like there is one special case where a problem. How can you convince the reader that the problem is more general (and therefore important to solve)?}

It is evident that, when imitating ergonomic human behaviour in robotic systems, direct imitation may be unsuitable in many cases. This paper addresses the need for empirical work in \PbD with naive users and aims to establish the link when learning from behaviours that are ergonomic for both the human and robotic systems, while still meeting the demands of the task.\jm{\done{\atMH:The last sentence needs to be adapted depending on whether you are presenting the contribution as a new method, or as an empirical paper. If the latter, you cannot claim that the behaviour is being 'adapted', instead, you must argue why the empirical work is needed.}}

\mh{The arguments presented so far treat manipulability and ergonomics as equivalent concepts, but this is not convincing - does anyone apart from you see them as equivalent? You need to either make a stronger link between the two (\cite{Jacquier-Bret2011} may help with this, but you need to properly argue the case), or find a way to make a more general argument about imitating ergonomic behaviour and use manipulability as a case study.}

%On the robots side, this work considers the control of systems taught using \PbD with non-expert users where demonstrations are subject to uncertain constraints, and also the need to optimise joint configurations based on the systems manipulability, which lead to greater degrees of freedom to flexibly perform demonstrated tasks.

%While both RULA and the manipulablity index can assess static poses, they differ in terms of ideal postures as shown in figure \fref{staticPosture}. This figure shows that the presented posture would score highly in RULA with 2 points which according to the RULA worksheet (\fref{reducedRulaImage}) is considered an acceptable posture and is thus ergonomic. However, when using the manipulability measure on the same pose, it is evident that obtaining a score of 0 in this case indicates that this posture is a singular pose, which for a system can lead to unpredictable and potentially dangerous behaviour. Therefore, in order to satisfy both the demonstrator and robot, it is necessary to allow the user to demonstrate the task according to their own comfort and then to adapt the ergonomic postures to that of the systems manipulability.

%\subsection{Example: Opening Drawers}\label{s:hose_Attachment}
%\begin{figure}[t!]
%      \centering%
% \includegraphics[width=0.48\textwidth]{images/constraintDrawerCartoonV4.png}
%      \caption{Demonstrating the task where the task space component shows reaching the drawer in various poses and a null space component of opening it subject to its linear constraint.}
%      \label{f:PbDRobotTask}
%\end{figure}  
%\noindent As a real world example, consider placing the robot in an environment designed for use by people such as an office. A robot trained to assist staff with, for example, collecting documents needs to be able to perform tasks such as reaching for and opening filing cabinets. In this case, the problem of teaching the robot to open and close drawers can be solved through \PbD (as shown in \fref{PbDRobotTask}). Programming by demonstration is suitable because office staff can decide to retrain systems when required in another office or if the room layout changes without having any expert knowledge of the system and the need to call in a specialist. The task policy is to have the demonstrators reach towards the drawer, after which the constraint matrix $\bA$ is determined by a linear constraint following the direction of the drawer opening.
%
%Where the task is directly demonstrated by the user or multiple users facing a filing cabinet, they might demonstrate the task from reaching towards a random point on the handle to opening the drawer towards themselves, and repeating this action multiple times using different starting points. In this scenario, the \textit{constraint} might be learnt in a straightforward manner using one of several constraint learning methods (see \sref{learningTheConstraint}).
%
% Unless explicitly instructed, however, the user might not take specific care of how the motion appears when performing those demonstrations. It can be assumed that the user performs demonstrations in a way which is  most comfortable for themselves, and this can be approximated using RULA.
%%For example, the user might choose to move towards and grab the drawer from the nearest point or in a pose/grip which allows demonstrations in the most comfortable manner for the user. 
%It is unlikely that an average user will know to avoid unstable or singular configurations---however, these may occur in various task-dependant situations. If, for example, a system placed in front of a drawer starts with all the joints fully extended, and a novice user then directs it to open the drawer by moving the arm directly back towards itself without resolving redundancy in the joint space, the system may propel itself in unpredictable directions due to the singularity. Moreover, systems that use an \textit{ad hoc} way of dealing with singularities, such as when using Matlab's pseudoinverse function which replaces singular values with zero are not satisfactory, as this prevents any movement of the system and thus comes at the expense of completing the task. A better way to do this is by maximising the system's manipulability.  


%\subsection{Task Manipulability and Programming by Demonstration}\label{s:manipulability-pbd}
%\noindent To avoid these problems and reduce uncertainty of encountering unstable or singular configurations (\sref{hose_Attachment}), traditionally, Yoshikawa's manipulability index is used, whereby the null space degrees of freedom are used to maximise the distance from singular points during the execution of the primary task.
%
%The manipulability is a measure of a system's ability to position and orientate its end-effector. In order to help with the designing and control of systems, Yoshikawa developed the manipulability index \cite{yoshikawa1984analysis}. It works by finding the linear dependencies in the task Jacobian which could result in reaching a singular configuration. Thus the following measure is used to assess manipulability
%\begin{equation}
%\v(\bx) = \sqrt{\det\left(\bA(\bx)\bA(\bx)^\T\right)}. \label{e:manipulability-index-with-A}
%\end{equation}
%\noindent Note that, \textit{computation of the manipulability presupposes the availability of $\bA$ in analytical form}---however, as noted in \sref{taskPioritisedConstraints}, this is usually unavailable in the context of \PbD where the primary task and associated constraints are \emph{implicit in the demonstrations}.
%
%As $\v\to 0$, the manipulability index indicates that the system is approaching a singular pose. The upper limit of $\v$ depends on the system itself and can only be provided once the entire work space is assessed (however the proposed method does not require this as it compares its manipulability locally). One of the applications of $\v$ lies in its use as a cost function to replace $\bpi$ in \eref{problem-solution} which results in the secondary task moving the system towards the goal using a path which favours higher manipulability (see \sref{constrainedV}).
%
%To obtain $\v$, such that it can be used in such a manner, this paper proposes to \emph{form an estimate of the constraints in a task and derive an estimate of \eref{manipulability-index-with-A}}. The approach uses demonstration data such that it is applicable even for non-experts with no formal knowledge of the constraints involved in a task. %In doing so, it allows for the robot to more accurately manoeuvre towards targets while minimising the risk of crossing over singular points and avoiding potentially unstable, unpredictable behaviour.
%
%\jm{\done{\atMH:\sref{problem_definition} is to do.}}


